Universality in Non-Equilibrium Quantum Systems

The phenomenon of universality is one of the most striking in many-body physics. Despite having sometimes wildly different microscopic constituents, systems can nonetheless behave in precisely the same way, with only the variable names interchanged. The canonical examples are those of liquid boiling into vapor and quantum spins aligning into a ferromagnet; despite their obvious differences, they nonetheless both obey quantitatively the same scaling laws, and are thus in the same universality class. Remarkable though this is, universality is generally a phenomenon limited to thermodynamic equilibrium, most commonly present at transitions between different equilibrium phases. Once out of equilibrium, the fate of universality is much less clear. Can strongly non-equilibrium systems behave universally, and are their universality classes different from those familiar from equilibrium? How is quantum mechanics important? This dissertation attempts to address these questions, at least in a small way, by showing and analyzing universal phenomena in several classes of non-equilibrium quantum systems.

==> endmatter/colophon.tex <==
%!TEX root = ../dissertation.tex
\newpage
\thispagestyle{empty}

% If you do want an image in the colophon:
\begin{figure}
  \vspace{20pt}
  \centering
  \hspace*{-32pt}
  \includegraphics[width=0.42\textwidth]{endmatter/colophon_hokusai.png}
\end{figure}

% If you don't want an image in the colophon:
% \vspace*{200pt}

\begin{center}
\parbox{300pt}{\lettrine[lines=1,slope=-2pt,nindent=-4pt]{\textcolor{SchoolColor}{T}}{his thesis was typeset} using \LaTeX, originally developed by Leslie Lamport and based on Donald Knuth's \TeX. A template that can be used to format a PhD dissertation with this look \textit{\&} feel has been released under the permissive \textsc{agpl} license, and can be found online at \href{https://github.com/suchow/Dissertate}{github.com/suchow/Dissertate} or from its lead author, Jordan Suchow, at \href{mailto:suchow@post.harvard.edu}{suchow@post.harvard.edu}. That template has been brought into accordance with the quirks of the \href{https://grad.berkeley.edu/academic-progress/dissertation/}{UC Berkeley dissertation guidelines} by the author. The above image is Hokusai's ``Great Wave off Kanagawa'', edited by the author. This rendition is in the \href{https://commons.wikimedia.org/wiki/File:Tsunami_by_hokusai_19th_century.jpg}{public domain}.   
}
%The body text is set in 11 point Egenolff-Berner Garamond, a revival of Claude Garamont's humanist typeface. The above illustration, \textit{Science Experiment 02}, was created by Ben Schlitter and released under \href{http://creativecommons.org/licenses/by-nc-nd/3.0/}{\textsc{cc by-nc-nd 3.0}}. 
\end{center}


==> frontmatter/abstract.tex <==
%!TEX root = ../dissertation.tex
% the abstract

\noindent The phenomenon of universality is one of the most striking in many-body physics. Despite having sometimes wildly different microscopic constituents, systems can nonetheless behave in precisely the same way, with only the variable names interchanged. The canonical examples are those of liquid boiling into vapor and quantum spins aligning into a ferromagnet; despite their obvious differences, they nonetheless both obey quantitatively the same scaling laws, and are thus in the same universality class. Remarkable though this is, universality is generally a phenomenon limited to thermodynamic equilibrium, most commonly present at transitions between different equilibrium phases. Once out of equilibrium, the fate of universality is much less clear. Can strongly non-equilibrium systems behave universally, and are their universality classes different from those familiar from equilibrium? How is quantum mechanics important? This dissertation attempts to address these questions, at least in a small way, by showing and analyzing universal phenomena in several classes of non-equilibrium quantum systems. \\ \vspace{12pt}

\noindent Chapter~\ref{introduction} begins with an introduction to the principle of universality, seen through the lens of Landau's theory of symmetry-breaking order parameters and phase transitions. It then covers the paradigmatic understanding of equilibrium universality via the set of ideas known as the renormalization group. Moving out of equilibrium, we discuss Floquet theory and periodically driven systems, before finally mentioning other examples of non-equilibrium universality as context for our later results. \\ \vspace{12pt}

\noindent Chapter~\ref{ch:CFT} investigates quantum critical systems described by a conformal field theory (CFT) driven at their boundary, both periodically in time and via noise. In the time-periodic case, we find that the system displays multiple dynamical regimes depending on the drive frequency.  We compute the behavior of quantities including the entanglement entropy and Loschmidt echo, confirming analytic predictions from field theory by exact numerics on the transverse field Ising model, and demonstrate universality by adding non-integrable perturbations. The dynamics naturally separate into three regimes: a slow-driving limit, which has an interpretation as multiple quantum quenches with amplitude corrections from CFT; a fast-driving limit, in which the system behaves as though subject to a single quantum quench; and a crossover regime displaying heating. The universal Floquet dynamics in all regimes can be understood using a combination of boundary CFT and Kibble-Zurek scaling arguments. We then move on to stochastic boundary driving. We formulate a generic ansatz for the dynamical scaling form of the typical Loschmidt echo and corroborate it with exact numerical calculations in the case of a spin impurity driven by shot noise in a quantum  Ising chain. We find that due to rare events the dynamics of the mean echo can follow very different dynamical scaling than the typical echo for certain classes of drives. Our results are insensitive to irrelevant perturbations of the bulk critical model and apply to all the microscopic models in the same universality class. \\ \vspace{12pt}

\noindent Chapter~\ref{ch:RSRG} considers disordered driven quantum systems, in particular, periodically driven (Floquet) systems that undergo many-body localization (MBL). We study transitions between distinct phases of one-dimensional Floquet systems. We argue that these are generically controlled by infinite-randomness fixed points of a strong-disorder renormalization group procedure. Working in the fermionic representation of the prototypical Floquet Ising chain, we leverage infinite randomness physics to provide a simple description of Floquet (multi)criticality in terms of a new type of domain wall associated with time-translational symmetry-breaking and the formation of `Floquet time crystals'. We validate our analysis via numerical simulations of free-fermion models sufficient to capture the critical physics. We then introduce a real-space renormalization group approach for Floquet MBL systems, asymptotically exact in the strong-disorder limit, and exemplify its use on the periodically driven interacting quantum Ising model. We analyze the universal physics near the critical lines and multicritical point of this model, and  demonstrate the robustness of our results to the inclusion of weak interactions. \\ \vspace{12pt}

\noindent Chapter~\ref{ch:Hydro} pivots to consider quantum effects in the context of hydrodynamics, in particular examining the phenomenon of Coulomb drag as a quantum analogue of the shear viscosity. Two conducting quantum systems coupled only via interactions can exhibit the phenomenon of Coulomb drag, in which a current passed through one layer can pull a current along in the other. As a transport signature, Coulomb drag has been found to be a sensitive probe of the systems' microscopic structure and displays a rich dependence with temperature. However, in quantum systems with particle-hole symmetry -- for instance, the half-filled Hubbard model or graphene near the Dirac point -- the Coulomb drag effect is vanishingly small. We point out that its {\it thermal} analogue, whereby a thermal current in one layer pulls a thermal current in the other, is nonzero at these particle-hole symmetric points and is indeed the dominant form of drag in particle-hole symmetric systems. By studying a quantum quench in the paradigmatic one-dimensional Hubbard model, we show that thermal drag, in marked contrast to charge drag, displays a non-Fermi's Golden Rule growth at short times due to a logarithmic scattering singularity generic to one dimension. Exploiting the integrability of the Hubbard model, we obtain the long-time limit of the quench for weak interactions. Finally, we connect these results to a thermal drag conductivity $\kappa_D$ via an appropriate Kubo formula, and comment on thermal drag effects in two-dimensional systems. \\ \vspace{12pt}

\noindent In Chapter~\ref{conclusion}, we close with comments on future lines of investigation, and on likely routes to a full understanding of non-equilibrium universality. 

%%%% plain-text 
%The phenomenon of universality is one of the most striking in many-body physics. Despite having sometimes wildly different microscopic constituents, systems can nonetheless behave in precisely the same way, with only the variable names interchanged. The canonical examples are those of liquid boiling into vapor and quantum spins aligning into a ferromagnet; despite their obvious differences, they nonetheless both obey quantitatively the same scaling laws, and are thus in the same universality class. Remarkable though this is, universality is generally a phenomenon limited to thermodynamic equilibrium, most commonly present at transitions between different equilibrium phases. Once out of equilibrium, the fate of universality is much less clear. Can strongly non-equilibrium systems behave universally, and are their universality classes different from those familiar from equilibrium? How is quantum mechanics important? This dissertation attempts to address these questions, at least in a small way, by showing and analyzing universal phenomena in several classes of non-equilibrium quantum systems. 
%
%Chapter 1 begins with an introduction to the principle of universality, seen through the lens of Landau's theory of symmetry-breaking order parameters and phase transitions. It then covers the paradigmatic understanding of equilibrium universality via the set of ideas known as the renormalization group. Moving out of equilibrium, we discuss Floquet theory and periodically driven systems, before finally mentioning other examples of non-equilibrium universality as context for our later results. 
%
%Chapter 2 investigates quantum critical systems described by a conformal field theory (CFT) driven at their boundary, both periodically in time and via noise. In the time-periodic case, we find that the system displays multiple dynamical regimes depending on the drive frequency.  We compute the behavior of quantities including the entanglement entropy and Loschmidt echo, confirming analytic predictions from field theory by exact numerics on the transverse field Ising model, and demonstrate universality by adding non-integrable perturbations. The dynamics naturally separate into three regimes: a slow-driving limit, which has an interpretation as multiple quantum quenches with amplitude corrections from CFT; a fast-driving limit, in which the system behaves as though subject to a single quantum quench; and a crossover regime displaying heating. The universal Floquet dynamics in all regimes can be understood using a combination of boundary CFT and Kibble-Zurek scaling arguments. We then move on to stochastic boundary driving. We formulate a generic ansatz for the dynamical scaling form of the typical Loschmidt echo and corroborate it with exact numerical calculations in the case of a spin impurity driven by shot noise in a quantum  Ising chain. We find that due to rare events the dynamics of the mean echo can follow very different dynamical scaling than the typical echo for certain classes of drives. Our results are insensitive to irrelevant perturbations of the bulk critical model and apply to all the microscopic models in the same universality class.
%
%Chapter 3 considers disordered driven quantum systems, in particular, periodically driven (Floquet) systems that undergo many-body localization (MBL). We study transitions between distinct phases of one-dimensional Floquet systems. We argue that these are generically controlled by infinite-randomness fixed points of a strong-disorder renormalization group procedure. Working in the fermionic representation of the prototypical Floquet Ising chain, we leverage infinite randomness physics to provide a simple description of Floquet (multi)criticality in terms of a new type of domain wall associated with time-translational symmetry-breaking and the formation of `Floquet time crystals'. We validate our analysis via numerical simulations of free-fermion models sufficient to capture the critical physics. We then introduce a real-space renormalization group approach for Floquet MBL systems, asymptotically exact in the strong-disorder limit, and exemplify its use on the periodically driven interacting quantum Ising model. We analyze the universal physics near the critical lines and multicritical point of this model, and  demonstrate the robustness of our results to the inclusion of weak interactions.
%
%Chapter 4 pivots to consider quantum effects in the context of hydrodynamics, in particular examining the phenomenon of Coulomb drag as a quantum analogue of the shear viscosity. Two conducting quantum systems coupled only via interactions can exhibit the phenomenon of Coulomb drag, in which a current passed through one layer can pull a current along in the other. As a transport signature, Coulomb drag has been found to be a sensitive probe of the systems' microscopic structure and displays a rich dependence with temperature. However, in quantum systems with particle-hole symmetry -- for instance, the half-filled Hubbard model or graphene near the Dirac point -- the Coulomb drag effect is vanishingly small. We point out that its thermal analogue, whereby a thermal current in one layer pulls a thermal current in the other, is nonzero at these particle-hole symmetric points and is indeed the dominant form of drag in particle-hole symmetric systems. By studying a quantum quench in the paradigmatic one-dimensional Hubbard model, we show that thermal drag, in marked contrast to charge drag, displays a non-Fermi's Golden Rule growth at short times due to a logarithmic scattering singularity generic to one dimension. Exploiting the integrability of the Hubbard model, we obtain the long-time limit of the quench for weak interactions. Finally, we connect these results to a thermal drag conductivity via an appropriate Kubo formula, and comment on thermal drag effects in two-dimensional systems.

%In Chapter 5, we close with comments on future lines of investigation, and on likely routes to a full understanding of non-equilibrium universality. 


==> frontmatter/dedication.tex <==
%!TEX root = ../dissertation.tex
% dedication text

To my family, past and future. 

==> frontmatter/previousworks.tex <==
Portions of the following previously published works by the author of this dissertation (``William Virgil Berdanier") appear in this dissertation:

\begin{itemize}
\item W. Berdanier, T. Scaffidi and J. E. Moore. ``Energy Drag in Particle-Hole Symmetric Systems as a Quantum Quench.'' \href{https://doi.org/10.1103/PhysRevLett.123.246603}{\textit{Phys. Rev. Lett.}, \textbf{123}, 246603 (2019)}. \href{https://arxiv.org/abs/1909.05251}{arXiv:1909.05251} \\
\item W. Berdanier, J. Marino and E. Altman. ``Universal Dynamics of Stochastically Driven Quantum Impurities.'' \href{https://doi.org/10.1103/PhysRevLett.123.230604}{\textit{Phys. Rev. Lett.}, \textbf{123}, 230604 (2019)}. \href{https://arxiv.org/abs/1906.11253}{arXiv:1906.11253} \\
\item {W. Berdanier}, M. Kolodrubetz, S. A. Parameswaran and R. Vasseur. ``Strong-Disorder Renormalization Group for Periodically Driven Systems." \href{https://doi.org/10.1103/PhysRevB.98.174203}{\textit{Phys. Rev. B}, \textbf{98}, 174203 (2018)}. \href{https://arxiv.org/abs/1807.09767}{arXiv:1807.09767}  \\
\item {W. Berdanier}, M. Kolodrubetz, S. A. Parameswaran and R. Vasseur. ``Floquet Quantum Criticality." \href{https://doi.org/10.1073/pnas.1805796115}{\textit{Proc. Natl. Acad. Sci.} \textbf{115} (38) 9491-9496 (2018)}. \href{https://arxiv.org/abs/1803.00019}{arXiv:1803.00019} \\
\item {W. Berdanier}, M. Kolodrubetz, R. Vasseur and J. E. Moore. ``Floquet Dynamics of Boundary-Driven Systems at Criticality." \href{https://doi.org/10.1103/PhysRevLett.118.260602}{\textit{Phys. Rev. Lett.} \textbf{118}, 260602 (2017)}. \href{https://arxiv.org/abs/1701.05899}{arXiv:1701.05899} \\
\end{itemize}

\nocite{PhysRevLett.123.246603,PhysRevLett.118.260602,Berdanier201805796,PhysRevB.98.174203,PhysRevLett.123.230604}

==> frontmatter/thanks.tex <==
%!TEX root = ../dissertation.tex
% the acknowledgments section

Well, it's been a wild ride. From my first exposure to physics through science fairs as a kid, to undergraduate research, two years in England and finally the past five years of grad school, this dissertation has been a long time coming. Thinking back, I'm both amazed by and grateful for all the help and joy I've received along the way.

First, I'd like to thank my advisor Joel Moore. I feel truly lucky to have had such a kind and generous mentor, whose research style and personality meshed well with my own. Blending quick wit with sharp insights, our numerous research discussions over the years have been illuminating and, more importantly, a lot of fun. I hope some of his physics intuition has rubbed off! More personally, from applying to fellowships early in grad school, to going to conferences and summer schools at the KITP and Les Houches, Joel has been my champion, and no doubt had a large hand in my successes. I'm also grateful for his help in this latest stage of my career, and for his support of my decision to take a new path. Thanks also to Ehud Altman, who has been like a second advisor to me. Ehud has a brilliant way of seeing which aspects of a problem are important and which are just details, and collaborating with him has taught me so much. Finally, thanks too to Birgitta for serving on my committee. 

It's almost impossible not to enjoy being at Berkeley. After all, even when research is going slowly and the stress is piling up, the sun is still shining brightly and the boba is nice and cold. Berkeley attracts wonderful people, both supremely talented and kindhearted. It's been a pleasure getting to know my fellow Moore-ons, Dan and Vir, as well as the Harvard-flung Dan Borgnia, as we've journeyed through grad school together. I've probably learned more from our discussions than from any coursework I took here. I'm also glad that the competitive nature of grad school never eclipsed our friendships, and that we were always willing to help one another, be it with presentations, coding, physics questions or simply life advice. I'm also greatly indebted to those older students in the group who kindly imparted their wisdom to me, from Philipp and Yasaman in my early years, to Byungmin and Aaron later on -- I hope I've been able to do the same for the younger generation. Aaron in particular deserves thanks, for being a total nerd with me. I look back fondly on our completely non-research-related conversations about video games, and learning Japanese together was a blast. Thanks also to Dragos for fun times playing softball and his constant politics-related needling, and to Illan for simply being a good friend. The culture at Berkeley is shaped by its incredible postdocs, and I feel utterly privileged to have worked with Romain Vasseur, Thomas Scaffidi and Mike Kolodrubetz. Thanks to Sid Parameswaran for hosting me at Oxford while we worked out the secrets of Floquet systems, and to Jamir Marino for hosting me later on at Harvard. 

One of the advantages of dating another scientist is getting looped into their large network of labmates and friends; thanks to all of the Gan lab members, including Marcus, Faten and David, for letting me crash their trivia nights (go Team Schwifty). Thanks also to my dear music (and hiking) friends, in particular Lynn, Eitan and Elyse, for filling my life with beautiful quartet experiences these past years. Here's to many more. 

Going to England was one of the most transformative experiences of my life. Thanks to Hanna, Christian and \'Alvaro for the wonderful times at Oxford during my brief refuge from physics in the world of philosophy; I'm glad we were able to meet up again in Chile. Thanks also to Dylan for keeping my physics skills sharp! Trite as it sounds, the greatest benefit of the Marshall was befriending the other people on it. Meeting so many brilliant people at the top of their fields, often of no relation whatsoever to physics, was a treat. Thanks to the Chads of the Flex (Bryan, Rahul, Shea, Jerod and Teddy) for a bunch of fun trips, and to Ben specifically for always being up for discussing topological insulators -- in addition to being one of the most caring and intelligent people I've ever met. My time at Cambridge was made so much richer by my musical friends in String Theory -- Kin, Franca, Jozefien, Philip, Agust\'in, and Jumpei. I'll always cherish the memories of playing for May Balls, performing in those glorious ancient chapels, and recording Brahms at Churchill. It's wonderful that we've been able to keep in touch, whether in Uruguay or Los Angeles, and I'm greatly looking forward to our next reunion. 

It all started in the Dean's Scholars program at UT Austin. Thanks to Nalin, Darius and Linhao for being three of my best friends these past ten years. It's been amazing witnessing your successes, and with two of you already in the C-suite, I promise to give you plenty of crap to keep your egos in check. Thanks too to my undergraduate mentors, Sacha Kopp and Gennady Shvets. Thanks Dr. Kopp for all of the help and support as I pursued the Marshall, and to Dr. Shvets for welcoming a know-nothing freshman into your research group. My summer at the Princeton Plasma Physics Lab inspired me to pursue physics in graduate school, and for that I thank Dr. Igor Kaganovich. Thanks to Albert for making that sweltering summer in rather dull Princeton fun, and a real adventure. 

Finally, thank you to my parents, Barry and Pam. No child can ever pay back the debt they owe, but I hope that I've been able to make you proud. Thank you to my grandparents, too, for always believing in me and supporting me. Thank you most of all to Lay, my brilliant, beautiful, hilarious stand-partner-for-life. I am so thrilled that we are finally married, and despite all the challenges we've faced, I know we have so much more `\emph{shiawase} together' in store. \emph{Daisuki da yo!}
